Categorifying Quiver Linking/Unlinking using CoHA Modules

The knots-quivers correspondence is a relation between knot invariants and enumerative invariants of quivers, which in particular translates the knot operations of linking and unlinking to a certain mutation operation on quivers. In this paper we show that the moduli spaces of a quiver and its linking/unlinking are naturally related, giving a purely representation theoretic interpretation of these operations. We obtain a relation between the cohomologies of these spaces which is moreover compatible with a natural action of the Cohomological Hall Algebra. The result is a categorification of quiver linking/unlinking at the level of CoHA modules.

==> xdasharrows.tex <==
\makeatletter
\newcommand*{\da@rightarrow}{\mathchar"0\hexnumber@\symAMSa 4B }
\newcommand*{\da@leftarrow}{\mathchar"0\hexnumber@\symAMSa 4C }
\newcommand*{\xdashrightarrow}[1][]{
  \mathrel{
    \mathpalette{\da@xarrow{}{#1}{}\da@rightarrow{\,}{}}{}%
  }
}
\newcommand{\xdashleftarrow}[1][]{
  \mathrel{
    \mathpalette{\da@xarrow{}{#1}\da@leftarrow{}{}{\,}}{}%
  }
}
\newcommand*{\da@xarrow}[7]{
  % #1: below
  % #2: above
  % #3: arrow left
  % #4: arrow right
  % #5: space left 
  % #6: space right
  % #7: math style 
  \sbox0{$\ifx#7\scriptstyle\scriptscriptstyle\else\scriptstyle\fi#5#1#6\m@th$}
  \sbox2{$\ifx#7\scriptstyle\scriptscriptstyle\else\scriptstyle\fi#5#2#6\m@th$}
  \sbox4{$#7\dabar@\m@th$}
  \dimen@=\wd0 
  \ifdim\wd2 >\dimen@
    \dimen@=\wd2 
  \fi
  \count@=2 
  \def\da@bars{\dabar@\dabar@}
  \@whiledim\count@\wd4<\dimen@\do{
    \advance\count@\@ne
    \expandafter\def\expandafter\da@bars\expandafter{
      \da@bars
      \dabar@ 
    }
  } 
  \mathrel{#3}
  \mathrel{ 
    \mathop{\da@bars}\limits
    \ifx\\#1\\
    \else
      _{\copy0}
    \fi
    \ifx\\#2\\
    \else
      ^{\copy2}
    \fi
  }
  \mathrel{#4}
}
\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../"
%%% End:

